Closed-book Question Generation via Contrastive Learning

Question Generation (QG) is a fundamental NLP task for many downstream applications. Recent studies on open-book QG, where supportive answer-context pairs are provided to models, have achieved promising progress. However, generating natural questions under a more practical closed-book setting that lacks these supporting documents still remains a challenge. In this work, we propose a new QG model for this closed-book setting that is designed to better understand the semantics of long-form abstractive answers and store more information in its parameters through contrastive learning and an answer reconstruction module. Through experiments, we validate the proposed QG model on both public datasets and a new WikiCQA dataset. Empirical results show that the proposed QG model outperforms baselines in both automatic evaluation and human evaluation. In addition, we show how to leverage the proposed model to improve existing question-answering systems. These results further indicate the effectiveness of our QG model for enhancing closed-book question-answering tasks.

==> few-shot-figures/eli5.tex <==
\begin{tikzpicture}[scale=0.7]
\begin{axis}[
    xlabel={Training Percentage (\%)},
    ylabel={RougeL},
    xmin=0, xmax=10,
    ymin=20, ymax=65,
    %ytick={60,65,70,75,80,85,90,95},
    legend pos=south east,
    legend style={fill=none},
    ymajorgrids=true,
    grid style=dashed,
]
\addplot+[
    thick,
    % color=yrbL1,
    mark=triangle,
    ]
    coordinates {
    (0,28.80)(1,32.32)(2,35.58)(3,38.55)(4,41.91)(5,41.91)(6,41.91)(7,41.91)(8,41.91)(9,41.91)(10,41.91)
    };
\addplot+[
    thick,
    % color=yrbL0,
    mark=square,
    ]
    coordinates {
    (0,28.80)(1,32.32)(2,35.58)(3,38.55)(4,41.91)(5,41.91)(6,41.91)(7,41.91)(8,41.91)(9,41.91)(10,41.91)
    };
\legend{BART-base, QG (ours)}
\end{axis}
\end{tikzpicture}

==> few-shot-figures/gooaq.tex <==
\begin{tikzpicture}[scale=0.45]
\begin{axis}[
    xlabel={Training Percentage (\%)},
    ylabel={RougeL},
    xmin=0, xmax=10,
    ymin=20, ymax=65,
    %ytick={60,65,70,75,80,85,90,95},
    legend pos=south east,
    legend style={fill=none},
    ymajorgrids=true,
    grid style=dashed,
    label style={font=\Large},
]
\addplot+[
    thick,
    % color=yrbL1,
    mark=triangle,
    ]
    coordinates {
    (0,28.80)(1,32.32)(2,35.58)(3,38.55)(4,41.91)(5,41.91)(6,41.91)(7,41.91)(8,41.91)(9,41.91)(10,41.91)
    };
\addplot+[
    thick,
    % color=yrbL0,
    mark=square,
    ]
    coordinates {
    (0,28.80)(1,32.32)(2,35.58)(3,38.55)(4,41.91)(5,41.91)(6,41.91)(7,41.91)(8,41.91)(9,41.91)(10,41.91)
    };
\legend{BART-base, QG (ours)}
\end{axis}
\end{tikzpicture}

==> few-shot-figures/wikicqa.tex <==
\begin{tikzpicture}[scale=0.45]
\begin{axis}[
    xlabel={Training Percentage (\%)},
    ylabel={RougeL},
    xmin=0, xmax=10,
    ymin=20, ymax=65,
    %ytick={60,65,70,75,80,85,90,95},
    legend pos=south east,
    legend style={fill=none},
    ymajorgrids=true,
    grid style=dashed,
    label style={font=\Large},
]
\addplot+[
    thick,
    % color=yrbL1,
    mark=triangle,
    ]
    coordinates {
    (0,28.80)(1,32.32)(2,35.58)(3,38.55)(4,41.91)(5,41.91)(6,41.91)(7,41.91)(8,41.91)(9,41.91)(10,41.91)
    };
\addplot+[
    thick,
    % color=yrbL2,
    mark=square,
    ]
    coordinates {
    (0,28.80)(1,32.32)(2,35.58)(3,38.55)(4,41.91)(5,41.91)(6,41.91)(7,41.91)(8,41.91)(9,41.91)(10,41.91)
    };
\legend{BART-base, QG (ours)}
\end{axis}
\end{tikzpicture}

==> tex/abstract.tex <==
\begin{abstract}

Question Generation (QG) is a dual task of Question Answering (QA), which can be leveraged as a data augmentation strategy to create large-scale QA pairs to improve the performance of a QA model.
QG methods have achieved promising results on reading comprehension datasets under an \textit{open-book} setting to generate natural questions based on the answer-context pairs. However, QG under a \textit{closed-book} setting, which challenges models to generate questions without passages, remains unexplored.
In this work, we present a new \textit{closed-book} dataset with abstractive long answers and a novel contrastive question generator for the \textit{closed-book} Question Answering task to bridge this gap.
By introducing the contrastive learning module and the answer reconstruction component, the proposed QG model can not only outperform the baseline system in the QG task during automatic evaluation, but also achieves the highest average ratings during human evaluation in terms of relevance and correctness. 
When we pre-train a \textit{closed-book} QA model with the synthetic QA pairs generated from the proposed QG model, it achieves improved performance on both seen and unseen datasets, which further demonstrates the effectiveness of our approach for enhancing unsupervised QA.

%Automatic evaluation results show that our QG model outperforms the baseline system and in human evaluations, it achieves higher average ratings in terms of relevance and correctness.
%generated synthetic QA pairs, we obtain significant improvements on both seen and unseen datasets.
%We further evaluate our approach using unsupervised QA: our QG model is used to generate synthetic QA pairs from article summary data to train a QA model.
%By pre-training the closed-book QA model on our 200K generated synthetic QA pairs, we obtain significant improvements on both seen and unseen datasets.




% Closed-Book Question Answering, which challenges models to answer questions without passages, has recently gained lots of interest.
% Significant advances in Question Answering (QA) task have been achieved by fune-tuning the pre-trained language models on large amounts of labeled QA datasets. 
% However, for new domains, obtaining labeled training data is labor-expensive and time-consuming. 
% To solve this problem, synthetic data generation has achieved promising results in past work, but remains unexplored under closed-book setting.
% In this work, we present the synthetic data generation framework under closed-book setting.
% We present a new dataset to train our question generator and introduce contrastive learning into our QG model to learn better representation.
% We take each sentence in freely available article summary data as answer and transform it into question.


% The resulting synthetic QA pairs are used to train a Closed-Book QA model.
% which generates synthetic question-answer pairs from article summary to pre-train QA model. 
% As a critical component in synthetic data generation framework, we  to learn better question representation and present a new QA dataset to train it.

\end{abstract}

==> tex/acknowledgments.tex <==
\section*{Acknowledgements}

==> tex/analysis.tex <==
\section{Analysis}

\subsection{Ablation Study}

The contribution of each component in the proposed question generator is investigated in an ablation study on the WikiCQA dataset and the results are shown in Table~\ref{tab:ablation-results}.
CL${_t}$ denotes using target predictions (questions) as positive pairs, which is described in Section~\ref{subsubsec:cl}. We also explore its variant -- CL${_s}$, in which we feed the same input to the encoder with different dropouts to obtain the positive pairs~\cite{gao-etal-2021-simcse}. We find that the choice of CL${_t}$ is slightly better than CL${_s}$ in terms of most evaluation metrics. Combined with the QA module, the performance can be further improved. Thus, we can prove the effectiveness of our contrastive learning module and the design of our framework.

\begin{table}[htbp!]
\centering\small
\begin{tabular}{lccccccc}
\hline
\textbf{Models} & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} & \textbf{R-LSum}\\
\hline
QG (BART-base) & 48.39 & 26.84 & 46.08 & 46.16  \\
QG+CL$_{s}$ & 48.67 & 27.34 & 46.43 & 46.46 \\
QG+CL$_{t}$ & 48.72 & 27.26 & 46.33 & 46.41 \\
QG+CL$_{s}$+QA & \textbf{49.26} & 27.77 & 46.82 & 46.88 \\
QG+CL$_{t}$+QA & 49.22 & \textbf{27.79} & \textbf{46.98} & \textbf{47.08} \\
\hline
\end{tabular}
\caption{Ablation study of QG model on \textit{WikiCQA}.}
\label{tab:ablation-results}
\end{table}

% \subsection{Few-Shot Question Answering}
% We conduct experiments in a few-shot learning setting, in which a limited number of labeled QA examples from the training set are used to train the model. 
% We take the model trained with our synthetic QA data and the vanilla BART-base model. 
% These models are trained using progressively increasing amounts of labeled QA samples from WikiCQA, GooAQ-Snippet, and ELI5 and evaluated on corresponding validation sets.
% Figure~\ref{fig:few-shots} shows the results where with less than 10\% data.
% We find our approach performs better than the baselines, which demonstrate the efficacy of our approach under few-shot setting.

% \begin{figure}[htbp!]
% \centering
%   \begin{subfigure}[b]{0.45\linewidth}
%   \include{few-shot-figures/wikicqa}
%   \vspace{-1cm}
%   \caption{WikiCQA}
%   \label{tab:wikicqa_few_shots}
%   \end{subfigure}
%   \hspace{\fill}
%   \begin{subfigure}[b]{0.45\linewidth}
%   \include{few-shot-figures/gooaq}
%   \vspace{-1cm}
%   \caption{GooAQ}
%   \label{tab:gooaq_few_shots}
%   \end{subfigure}
%   \hspace{\fill}
% %   \begin{subfigure}[b]{0.25\textwidth}
% %   \include{few-shot-figures/eli5}
% %   \vspace{-0.5cm}
% %   \caption{ELI5}
% %   \label{tab:eli5_few_shots}
% %   \end{subfigure}
% %   \hspace{\fill}
% \caption{RougeL on test set by varying the proportions of
% training data (from 1\% to 10\%).}
% \label{fig:few-shots}
% \end{figure}

% 1, 2, 3, 4, 5, 6, 7, 8, 9, 10%

\subsection{Case Study}

Finally, we showcase some examples of the generated questions on the WikiCQA dataset. As Table~\ref{tab:good-examples} shows, our model can produce better questions than baseline.
For the first examples in Table~\ref{tab:good-examples}, we can see our model generates ``how many'' for the statistics-type answer, which is closer to the reference ``what percentage'' than the baseline model. For the second one, although the reference contains the detailed information ``textured surface'' which is not in the answer, our model captures the information ``without nails'', which is more informativeness than the baseline model.
There are also some cases where our model fails to generate good questions, which are shown in Table~\ref{tab:bad-examples}. 
Compared with the reference question ``what food can be included on a clear liquid diet'', our model generates ``what can I eat to lose weight'', which fails in automatic evaluation metrics and is hard for annotators to justify in terms of relevance. 
For the second one, although ``broken door'' which is generated from our model is relevant to the answer, it's still far from the reference ``door sticking to the weather strip''. The question generated from the baseline model which is related to ``bedroom'' is even worse in terms of relevance.


\begin{table}
\centering
\begin{subtable}{\linewidth}
\centering\small
\begin{tabular}{p{0.02\textwidth}p{0.85\textwidth}}
\hline
$\textbf{A}$ & The most recent statistics show that around 2.5\% of small businesses are audited by the irs. \\
$\textbf{Q}_{B}$ & Are small businesses audited by the irs? \\
$\textbf{Q}_{G}$ & How many small businesses are audited by the irs? \\
$\textbf{Q}_{R}$ & What percentage of small businesses are audited? \\ \hline
$\textbf{A}$ & Try using poster putty to secure the images in your collage. if that doesn't work, you may have to use nails. \\
$\textbf{Q}_{B}$ & How do i put pictures in a collage? \\
$\textbf{Q}_{G}$ & How do i make a collage without nails? \\
$\textbf{Q}_{R}$ & How can i make a collage on a wall with a textured surface? \\
\hline
\end{tabular}
\caption{Good examples.}
\label{tab:good-examples}
% \end{table}
\end{subtable}
\vspace{1ex}

% \begin{table}[hb!]
% \centering\small
\begin{subtable}{\linewidth}
% \begin{tabular}{p{0.25cm}p{0.4\textwidth}}
\centering\small
%\begin{tabular}{cl}
\begin{tabular}{p{0.02\textwidth}p{0.85\textwidth}}
\hline
$\textbf{A}$ & Foods such as popsicles, hard candy, and gelatin can be eaten on a clear liquid diet. \\
$\textbf{Q}_{B}$ & what can you eat on a clear liquid diet? \\
$\textbf{Q}_{G}$ & What can I eat to lose weight? \\
$\textbf{Q}_{R}$ & What food can be included on a clear liquid diet? \\ \hline
$\textbf{A}$ & You'll have to remove the door and sand, prime, and repaint it. \\
$\textbf{Q}_{B}$ & What do i have to do to make my bedroom look nice? \\
$\textbf{Q}_{G}$ & How do i fix a broken door? \\
$\textbf{Q}_{R}$ & What do i do if my door is sticking to the weather strip? \\
\hline
\end{tabular}
\caption{Bad examples.}
\label{tab:bad-examples}
\end{subtable}
\caption{Generated question examples. $\textbf{Q}_{B}$: generated questions from baseline model; $\textbf{Q}_{G}$: generated questions from our proposed QG model;
$\textbf{Q}_{R}$: reference questions.}
\label{tab:examples}
\vspace{-2ex}
\end{table}





==> tex/approach.tex <==
\section{Proposed Approach}
\label{sec:approach}

% Question and answer generation is a data augmentation method aiming to improve question answering (QA) models given the limited amount of human labeled data. 
% However, most prior work on question generation are performed on reading comprehension dataset, where the input is a question and context and the output is an answer.
% \citet{mishra-etal-2020-towards} The existing question generation model for long answers~\cite{} performed on extractive NQ~\cite{kwiatkowski-etal-2019-natural} dataset where the long answers are typically paragraphs from the relevant Wikipedia page.
% The closed-book question answering task challenges systems to answer questions without any additional information sources such as knowledge bases or evidence documents.
% As a result, models must solely rely on the question text and the information stored inside the model weights during training.
% In addition, generating questions from long-form answers is more challenging than detail-based questions. \textcolor{blue}{CAV: why? explain this a little more ... and by  "detail" I think you mean factoid style?}
% Our model needs to summarize the whole answer instead of based on extracted spans or entities from the paragraph. 

% \textcolor{blue}{CAV: really need a figure to walk through this whole workflow so it is clear.} In this work, we focus on this closed-book long-form question answering task where the goal is to answer a question without a supporting passage and propose our summary-based synthetic data generation pipeline to improve it.

Diverging from the current QG models under the open-book setting, we propose a closed-book QG model, which generates questions directly without context.
To improve the question representation, we integrate contrastive learning and answer reconstruction into it (Section~\ref{subsec:qg}).
Then the trained QG model is employed to generate synthetic QA pairs from a summary dataset which is used to pre-train an unsupervised QA model (Section~\ref{subsec:synthetic}).
% In our synthetic data generation pipeline, firstly, we trained QG model with labeled dataset. 


\begin{figure}[htbp!]
\centering
\includegraphics[width=\linewidth]{img/qg_model.pdf}
\caption{An overview of the proposed question generator, which consists of three parts: contrastive learning, question generation, and answer construction.}    
\label{fig:qg-framework}
\end{figure}


\subsection{Question Generator}
\label{subsec:qg}

As a dual task of closed-book QA task, the closed-book QG task aims to generate a natural question $y$ given an input answer sentence $x$.
Figure~\ref{fig:qg-framework} illustrates an overview of the proposed QG framework, which consists of three parts, contrastive learning, question generation, and answer reconstruction.
Our model is trained by optimizing three losses simultaneously.

\subsubsection{Question Generation}
\label{subsubsec:qg}

The system is based on the sequence-to-sequence architecture which consists of an encoder and a decoder ~\cite{sutskever-etal-2014-sequencetosequence,vaswani-etal-2017-attention}. 
The encoder takes an input sequence of source words $\textbf{x} = (x_1, x_2, \dots, x_n)$ and maps it to a sequence of continuous representations $\textbf{z} = (z_1, z_2, \dots, z_n)$. 
Then, the decoder takes $\textbf{z}$ and generates a sequence of target words $\textbf{y} = (y_1, y_2, \dots, y_m)$ at a time.
The QG task is defined as finding $\hat{y}$:
\begin{equation}
    \hat{\textbf{y}}=\underset{\textbf{y}}{\arg\max} p(\textbf{y}|\textbf{x}),
\end{equation}
where $p(\textbf{y}|\textbf{x})$ is the conditional log-likelihood of the predicted question sequence $\textbf{y}$ given input $\textbf{x}$.
\begin{equation}
    p(\textbf{y}|\textbf{x})=\prod_{i=1}^{T}p(y_{t}|\textbf{y}_{<t},\textbf{x}),
\end{equation}
% More detailed, at each time step $t$, the predicted probability $p_{t}$ of the $t$-th target word...  
% More detailed, at each time step t, the hidden state $h_{t}$ is updated by
% \begin{equation}
%     h_{t} = f(x_{t},h_{t-1}),
% \end{equation}
% where $x_{t}$ is the word embedding received by the encoder and $h_{t-1}$ is the previous hidden state.

Given answer-question pairs $\mathcal{S}=\left\{(x_{i}, y_{i})  \right\}_{i=1}^{n}$, the training objective of our model is to minimize the Negative Log-Likelihood (NLL) of training data,
\begin{equation}\label{eq:qg}
    \mathcal{L}_{qg}=-\sum_{i=1}^{N}\log p(q_{i}|A),
\end{equation}
where $q_{i}$ is the $i$-th token in the generated question and $A$ is the answer.

% \textcolor{blue}{CAV: is it worth mentioning the loss by name here $\mathcal{L}_{qg}$?}
To improve the sentence representation in the question generator, we introduce the contrastive learning and answer reconstruction modules next. 
% in Section~\ref{subsubsec:cl},~\ref{subsubsec:ar}.


\subsubsection{Contrastive Learning}
\label{subsubsec:cl}

To assist the encoder in our Question Generator to learn a better representation, we introduce the contrastive learning loss into our QG framework, with the objective to minimize the distance between positive pairs and maximize the distance between negative pairs~\cite{chen-etal-2020-simple}. Specifically, given a positive pair $\mathcal{S}=\left\{(x_{i}, x_{j})  \right\}_{i=1}^{n}$, the other $2(N-1)$ examples within a mini-batch are treated as negative examples. 

% $h_{i}$ and $h_{j}$ are the representations of $x_{i}$ and $x_{j}$, which 
With the aforementioned contrastive objective, how to construct the appropriate positive pairs is a critical problem.
In our work, aiming to learn better question representation and force the encoder to distinguish features of correct QA pairs from features of incorrect QA pairs, we take the ground-truth question as the positive instance of an answer and fine-tune the model parameters based on the contrastive loss function,
\begin{equation}\label{eq:cl}
    \mathcal{L}_{cl}=-\log\frac{\exp(\text{sim}(\textbf{z}_{i},\textbf{z}_{j})/\tau_{cl})}{\sum_{k=1}^{2N}\exp(\text{sim}(\textbf{z}_{i},\textbf{z}_{k})/\tau_{cl})},
\end{equation}
where $\textbf{z}$ is the representation of input sentences, $\text{sim}(\textbf{z}_{i},\textbf{z}_{j})=\textbf{z}_{i}^{\top}\textbf{z}_{j}/\left\| \textbf{z}_{i} \right\|\left\| \textbf{z}_{j} \right\|$ denotes cosine similarity, and $\tau_{cl}$ is a temperature parameter.
In this work, $\textbf{z}$ is the embedding of the special token $[CLS]$ from the transformer encoder, which represents the meaning of the entire sentence.
% by prepending the input sentence with special token $[CLS]$ and fed into the transformer encoder, which generates the sequence of embeddings, respectively.
% $e^{cls}$, which is the embedding of the special token, 
% We get the representations $\textbf{z}$ of input sentences $x$ via $\textbf{z}=f_{\theta}(x)$, where $f_{\theta}$ is an encoder from pre-trained language model (e.g., BART \cite{lewis-etal-2020-bart}).
% In our work, question and answer are prepended by the special token $[CLS]$ and fed into the transformer encoder, which generates the sequence of embeddings, respectively.
% $e^{cls}$, which is the embedding of the special token, 

% With the aforementioned contrastive objective, how to construct the appropriate positive pairs is a critical problem. The most direct approach is to editing the input text with operations such as random shuffling, replacing, deleting or substituting words~\cite{wei2019eda}. 
% However, directly modifying the sentences may affect their original semantic meaning \cite{gao-etal-2021-simcse}. 
% Thus, in our first setting, instead of editing the input sentences, we feed the same input to the encoder with different dropout to get two output embeddings, which can be regarded as the positive pairs with similar semantic meaning.
%\textcolor{blue}{CAV: need to say a bit more about what you do here ... why is this interesting? why is it a good idea?}

% Then the loss function for a mini-batch of $N$ examples becomes:
% \begin{equation}
%     \mathcal{L}_{cl}=-\log\frac{\exp(\text{sim}(\textbf{z}_{i},\textbf{z}_{i}^{'})/\tau_{cl})}{\sum_{k=1}^{N}\exp(\text{sim}(\textbf{z}_{i},\textbf{z}_{k})/\tau_{cl})}
% \end{equation}
% In our second setting, we take the target sentences as positive samples and fine-tune the parameters based on the same loss function as Equation~\ref{eq:1}. 
% \textcolor{blue}{CAV: same deal, need to explain why this is a good idea; how is it different than the previous method? (in other words, you do two approaches; what is the intuition or goal of them?)}


\subsubsection{Answer Reconstruction}
\label{subsubsec:ar}

A good question representation should have the ability to generate the original answer.
To measure the answerability of the generated question, we use a pre-trained seq2seq model to predict the original answer given the generated question. Like the closed-book QA model, the loss is calculated by a negative log likelihood loss function: 
\begin{equation}\label{eq:ar}
    \mathcal{L}_{ar}=-\sum_{i=1}^{N}\log p(a_{i}|Q)
\end{equation}
where $a_{i}$ is the $i$-th token in the answer and Q is the generated question.

% \textcolor{blue}{CAV: should you mention the loss here? and tell us a bit more about how it is measured?}
A major problem when passing the output from the QG part (Section~\ref{subsubsec:qg}) to the QA part is that the model is not fully differentiable.
Gradients cannot be back-propagated directly.
% Many previous works apply Reinforcement Learning (RL) due to the discreteness of language, such as machine translation~\cite{brakel-etal-2017-actor}, image captioning~\cite{rennie-etal-2017-self}, and abstractive summarization~\cite{paulus-etal-2018-deep}.
% However, suffering from high variance, RL is slow to converge.
In our work, instead of using RL, we employ the Straight-Through (ST) Gumbel-Softmax for gradient computation~\cite{jang-etal-2017-categorical}.
% \smallskip
% \noindent\textbf{Straight-Through Gumbel-Softmax}  
% In ST Gumbel-Softmax, the argmax function is replaced by the differentiable softmax function. 
The ST Gumbel-Softmax is a discrete version of the Gumbel-Softmax and takes different forward and backward paths. In the forward pass, the embedding is discretized by using the argmax, whereas in the backward pass the gradients are computed by the gumbel-softmax~\cite{qader-etal-2019-semi}. 
\begin{equation}
    y_{i} = \frac{\exp((\log(p_{i})+g_{i})/\tau_{gs})}{\sum_{j=1}^{|V|}\exp((\log(p_{j})+g_{j})/\tau_{gs})}
\end{equation},
where $\tau_{gs}$ is a temperature parameter and $g_{i}$ is the Gumbel noise drawn from a uniform distribution $(0,1)$. 
% When $\tau_{gs}\to0$, $y_{i}$ becomes the one hot representation. 
In our work, the one-hot embedding from ST Gumbel-Softmax is multiplied with the  vocabulary embedding and then fed into the encoder of the pre-trained seq2seq model as the initial representation of the generated question.
% \cite{goyal-etal-2017-differentiable} reports Straight-Through Gumbel-Softmax outperforms scheduled sampling and converges faster than reinforcement learning~\cite{havrylov-titov-2017-emergence}


\subsubsection{Overall Loss Function}
As a result, all three losses are summed together to provide the overall loss function $\mathcal{L}$ as follows:
\begin{equation}\label{eq:total}
    \mathcal{L} = \lambda_{1} \mathcal{L}_{qg} + \lambda_{2}\mathcal{L}_{cl} + \lambda_{3}\mathcal{L}_{ar}
\end{equation}
The weights $\lambda_{1}$,$\lambda_{2}$, and $\lambda_{3}$ are tuneable hyper-parameters to balance losses and the final objective is to minimize the overall loss.

The functionality of the whole QG framework is presented in Algorithm~\ref{alg:qa}. 
% \textcolor{blue}{CAV: need to update equation refs in the algorithm; also, sometimes we say answer-question pairs, and other times it is question-answer pairs -- does it matter?}

\begin{algorithm}[!ht]
\caption{Question generator.}
\label{alg:qa}
\SetKwInput{KwData}{Input}
\SetKwInput{KwResult}{Output}
\KwData{Pre-trained language model $p(q|a)$, QA model $p(a|q)$ and QA pairs}
\KwResult{Question generator $p(q|a)$}
\For{$i\gets1$ \KwTo $Epoch$}{
    $\hat{q} = p(q|a)$ \\
    Compute $\mathcal{L}_{qg}$ via Eq.~\ref{eq:qg} \\
    \tcc{contrastive learning}
    $a_i = \text{Encoder}([CLS]\oplus a)[:,0:]$ \\
    $a^{+}_{i} = \text{Encoder}([CLS]\oplus q)[:,0:]$ \\
    Get $\mathcal{L}_{cl}$ to $(a_i,a^{+}_{i})$ via Eq.~\ref{eq:cl} \\
    \tcc{answer reconstruction}
    $\hat{a} = p(a|\hat{q})$ \\
    Compute $\mathcal{L}_{ar}$ via Eq.~\ref{eq:ar} \\
    Calculate total loss $\mathcal{L}$ via Eq.~\ref{eq:total} \\
    Update generator $p(q|a)$ with $\mathcal{L}$}
\Return question generator $p(q|a)$
\end{algorithm}


\subsection{Synthetic QA Data Generation}
\label{subsec:synthetic}

% Recent approaches for synthetic QA data generation typically consist of multi-stages: answer extraction, question generation, and question filtering~\cite{alberti-etal-2019-synthetic, puri-etal-2020-training}.
% For a given passage, the responsibility of the answer extractor is to extract appropriate spans that will serve as answers to generate questions. 
% Usually, question (un)conditional extractive answer models~\cite{alberti-etal-2019-synthetic, puri-etal-2020-training} or heuristics (e.g., noun phrases, named entities)~\cite{lewis-etal-2019-unsupervised, lyu-etal-2021-improving} are used in this module.
% Then, they generate questions conditioned on passage and answer.
% After that, the questions are filtered based on the roundtrip consistency.
% To reduce the errors propagated from each module to others in the pipeline, \citet{shakeri-etal-2020-end} proposed an end-to-end approach for synthetic QA data generation.
% However, these work are all performed on Reading Comprehension dataset which is different from the closed-book long-form setting. \textcolor{blue}{CAV: need to talk about our naming conventions ... here it is "closed-book long-form" ... are we consistent? and we should carefully introduce what we mean by long form earlier in the paper (and contrast with the other kind ... the factoid/short kind, maybe with an example)}
% Since freely available summary data is a good resource to generate synthetic data~\cite{lyu-etal-2021-improving}, we explore the synthetic data generation for closed-book QA task based on the summary data.


We further evaluate our approach by generating synthetic data using our QG model and fine-tuning the unsupervised closed-book QA model.
As shown in Figure~\ref{fig:pipeline}, we take each sentence from the summary of an article as an answer and use our QG model, which is described in Section~\ref{subsec:qg}, to generate questions only conditioned on answers.
Then, we train an unsupervised QA model based on the synthetic QA pairs, which is optimized by the following negative log likelihood loss function:
\begin{equation}
    \mathcal{L}_{qa}=-\sum_{i=1}^{N}\log p(a_{i}|Q),
\end{equation}
where $a_{i}$ is the $i$-th token in the generated answer and Q is the question.

% \textcolor{blue}{CAV: how is this loss connected to the loss in the previous section? need to be clear.}


==> tex/conclusion.tex <==
\section{Conclusion}

In this work, we investigate improving closed-book Question Answering from a data augmentation perspective with Question Generation. We present a new closed-book dataset with abstractive long answers of more than 20K real user QA pairs. We introduce the contrastive learning objective and an answer reconstruction component, leading to a QG model which achieves better performance than baselines through both automatic and human evaluations.
Furthermore, we evaluate our approach by employing our QG model on article summary data to generate synthetic QA pairs, which are used to pre-train a closed-book QA model.
Our experiments show that the pre-trained QA model performs best on the seen dataset and shows strong generalization on unseen datasets, with or without further fine-tuning. %For the future work, we would explore other models to improve closed-book QA task.






==> tex/dataset.tex <==
\section{WikiCQA: A New Dataset}
\label{sec:dataset}

% We aim to perform synthetic QA data generation based on the summary of an article. 
% \textcolor{blue}{CAV: rather than contrast with other datasets, start out talking about the good things about our dataset. Why it is interesting. Why it is good. Then shift to compare to existing ones.}

In this section,  we introduce a new closed-book QA dataset called WikiCQA.% which can be used for question answering task in closed-book setting. 

% However, the existing long-form QA dataset, ELI5, which can be used for closed-book long-form QA task, only has the whole supporting documents.
% Although GooAQ dataset is constructed based on closed-book setting, we can not use it to further generate synthetic QA data.
% % unlike the reading comprehension setting, the context for answering the question is not provided as part of the input
% Instead of generating summaries from the supporting context~\cite{murakhovs-etal-2021-mixqg} which may introduce the errors from the summarization model, we introduce a new closed-book long-form QA dataset called WikiCQA, which can be used with WikiSum dataset~\cite{cohen-etal-2021-wikisum}, a user-generated article summary dataset from WikiHow, for our summary-based synthetic data generation.% which can be used for question answering task in closed-book setting. 

\subsection{Dataset Construction}

% \todo{TODO: add answer, ground truth question, generated questions examples on the right}
WikiHow\footnote{\url{https://www.wikihow.com}, under an Attribution-Noncommercial-Share Alike 3.0 Creative Commons License.} is a wiki-style website featuring over 200K how-to articles. 
We collect the question-answer pairs from the Q\&A section (or Expert QA, Question Answering under some documents) of articles on WikiHow to construct the dataset. 
The questions and answers are related to the specific articles, which are asked by WikiHow users and answered by a knowledgeable reader or editor\footnote{\url{https://www.wikihow.com/Use-wikiHow\#Reading-and-Learning-from-wikiHow}}. 
After removing duplicates and question-answer pairs with meaningless answers, 23,037 QA pairs remain. 
To keep the same format as other existing QA datasets (e.g., ELI5, GooAQ), we further discard questions not starting with a question-type word (e.g., what, how). 
% The full list of question terms is in Appendix~\ref{sec:question-type-unigram}. 
After the dataset processing steps, we arrive at 20,202 question-answer pairs.

In Table~\ref{tab:an-example}, we show an example article from Wikihow, which includes the title and summary of the article and question-answer pairs from the corresponding Q\&A section. From the example we can see answers in our dataset are abstractive long answers, which are written by real users and not contained within the context passage. These are different from the answers in reading comprehension datasets, where the answers are a short text span in the context.
 

\begin{table}[htbp!]
\centering\small
\begin{tabular}{p{0.45\textwidth}}
\hline
\textbf{Title:} How to Prepare a Healthy Meal for Your Pet Dog. \\
\textbf{Summary:} To prepare a healthy meal for your dog, choose lean meat with the bones and fat removed, like chicken or beef \dots \\ 
\textbf{Q:} What can I feed my dog if I have run out of dog food? \\
\textbf{A:} In the short term, any bland human food such as chicken or white fish with rice or pasta is just fine \dots \\
\textbf{Q:} How much homemade dog food do you feed your dog? \\
\textbf{A:} Great question because it highlights one of the problems of feeding home prepared foods \dots \\
\textbf{Q:} What should I not feed my dog?  \\
\textbf{A:} There are many human foods that are toxic to dogs. Top of the list of foods NOT to give are \dots \\

\hline
\end{tabular}
\caption{Question-answer pairs from WikiHow Q\&A section.}
\label{tab:an-example}
\end{table}


% \textcolor{blue}{CAV: somewhere in this section need to give some more explanation of how these answers are long-form; not just simple facts, but interesting, challenging answers. You give some examples, now tell us so we really appreciate it.}


\subsection{Dataset Analysis}
\label{subsec:dataset-analysis}

\begin{figure*}[htbp!]
\centering
    \begin{subfigure}[!]{0.20\textwidth}
    \include{data-analysis-figures/question-length}
    \vspace{-0.5cm}
    \caption{Question (Q) length.}
    \label{fig:question-length}
    \end{subfigure}
    \hspace{\fill}
    \begin{subfigure}[!]{0.30\textwidth}
    \include{data-analysis-figures/answer-length}
    \vspace{-0.5cm}
    \caption{Answer (A) length.}
    \label{fig:answer-length}
    \end{subfigure}
    \hspace{\fill}
    \begin{subfigure}[!]{0.45\textwidth}
    \include{data-analysis-figures/question-unigram}
    \vspace{-0.5cm}
    \caption{Common question-word.}
    \label{fig:question-unigram}
    \end{subfigure}
    \hspace{\fill}
 \caption{Comparison on the distribution of Q-A length and question types among three datasets.}    
\label{fig:data-analysis}
\end{figure*}


To better understand the content of WikiCQA in comparison with existing QA datasets, consider the three figures shown in Figure~\ref{fig:data-analysis}. 
We measure the length of each question or answer with the number of tokens returned from BART Tokenizer~\cite{lewis-etal-2020-bart}. 
Firstly, in Figure~\ref{fig:question-length} we compare the question length distribution for WikiCQA versus two existing QA datasets, which can also be used under the closed-book setting, GooAQ-S~\cite{khashabi-etal-2021-gooaq-open} and ELI5~\cite{fan-etal-2019-eli5}. 
%whosn in we present a series of observations. 
While more than 80\% of the questions in WikiCQA and GooAQ-S have less than 15 tokens, questions in ELI5 have a broader length range.
% \textcolor{blue}{CAV: need to update this.}
Second, we compare the answer length distribution for these datasets in Figure~\ref{fig:answer-length}, where we observe that more than 90\% of answers from WikiCQA and GooAQ-S lie in the range of 16-127 tokens, while ELI5 has a broader range of lengths.
Finally, to gain insights about the question type, we measure the proportion of the leading unigram that starts a question in Figure~\ref{fig:question-unigram}. 
The dominant pattern is ``how'' questions in WikiCQA while ELI5 has many ``why'' questions. 
Overall, our dataset WikiCQA also has a wide distribution of question types.


% To better understand the content of WikiCQA in comparison with existing QA datasets, consider the three figures shown in Figure~\ref{fig:data-analysis}. 
% In the first -- Figure~\ref{fig:question-length} -- we compare the question length distribution (question is tokenized by BART~\cite{lewis-etal-2020-bart} tokenizer)(\textcolor{blue}{HOW DO WE MEASURE LENGTH HERE?} for WikiCQA versus two existing long-form question answering datasets, GooAQ-Snippet~\cite{khashabi-etal-2021-gooaq-open} and ELI5~\cite{fan-etal-2019-eli5}. whosn in we present a series of observations. 
% While all the questions in GooAQ-Snippet have less than 15 tokens, questions in WikiCQA and ELI5 have broader length range.
% \textcolor{blue}{What do we learn from this figure? Add a sentence or two.} 
% Second, we compare the answer length distribution for these same datasets in Figure~\ref{fig:answer-length}, where we observe that majority of answers from WikiCQA and GooAQ-Snippet have 16-127 tokens, ELI5 has broader range of lengths.\textcolor{blue}{What do we learn from this figure? Add a sentence or two.}. 
% Finally, to gain insights about the question type, we measure the proportion of the leading unigram that starts a question in Figure~\ref{fig:question-unigram}. 
% The dominant pattern is 'how' questions in WikiCQA while ELI5 has many 'why' questions.  \textcolor{blue}{What do we learn from this figure? Add a sentence or two.}




==> tex/experiments.tex <==
\section{Experiments}

In this section, we conduct experiments of our proposed QG model over three datasets: WikiCQA, GooAQ-Snippet, and ELI5. Then we employ our best QG model on a WikiHow-based summary dataset (WikiSum) to generate the synthetic question-answer pairs to pre-train an unsupervised QA model, which is also evaluated on the same three datasets. It is worth noting that for the proposed QG model, the input sentences are answers and ground-truth sentences are questions from these three datasets; while for the QA model, the input and output are opposite.

% We use the new dataset WikiCQA for in-domain evaluation, and the two existing long-form question answer datasets, GooAQ-Snippet and ELI5, for out-of-domain evaluation in the long-form closed-book setting. For question answering task, we use a WikiHow-based summary dataset (WikiSum) to generate the synthetic question-answer pairs to pre-train the QA model, which is also evaluated on the WikiCQA, GooAQ-Snippet, and ELI5 datasets. It is worth-noting that, for the proposed QG model the input sentences are answers and ground-truth sentences are questions from these three dataset; while for the QA model, the input and output are opposite.  
%In this section, firstly, we describe the corpora and data split. Then, we give details of the model and experimental settings. At last, we introduce the evaluation metrics, following by the results.

\subsection{Data Split}
For our QG model, we adopt (1) \textbf{WikiCQA} dataset containing 20,202 QA pairs (as introduced in  Section~\ref{sec:dataset}). We shuffle the data and split it to train, validation, and test sets by the ratio of 80\%/10\%/10\%. 
(2) \textbf{GooAQ-S} is a sub-sampled dataset from GooAQ~\cite{khashabi-etal-2021-gooaq-open}. 
GooAQ contains three different sub-tasks: short, snippet (i.e., multi-sentence description), and collection response questions. 
Under the long-form closed-book setting, we adopt the snippet part (i.e., questions with snippet answers) for our experiments as in the original paper.
Furthermore, from the paper, the model performance on the snippet task does not vary much when supervised with 200K and 2M training instances. 
Thus, to improve the experimental efficiency, we take 200k instances from the snippet set and split them based on their original scripts.\footnote{\url{https://github.com/allenai/gooaq/blob/main/experiments/create\_splits.py}}
(3) \textbf{ELI5}~\cite{fan-etal-2019-eli5} is a widely-used large-scale corpus for long-form question answering with supporting web documents.
In this work, we only use the question-answer pairs from the dataset and ignore the supporting context to fit the closed-book setting here.
We follow the data split from huggingface.\footnote{\url{https://huggingface.co/datasets/eli5}}
The detailed data statistics and splits of the aforementioned datasets are shown in Table~\ref{tab:data-split}.

\begin{table}[t!]
\centering
\begin{tabular}{lrrr}
\hline
\textbf{Datasets} & \textbf{Train} & \textbf{Val} & \textbf{Test}\\
\hline
WikiCQA & 16,162 & 2,020 & 2,020 \\
GooAQ-S & 200,000 & 500 & 498 \\
ELI5 & 272,634 & 9,812 & 24,512 \\
\hline
\end{tabular}
\caption{Dataset Statistics.}
\label{tab:data-split}
\end{table}

To generate synthetic question-answer pairs, we use \textbf{WikiSum}~\cite{cohen-etal-2021-wikisum}, which is a dataset based on coherent-paragraph summaries written by the article's authors on the WikiHow website. It contains 39,775 summaries. 
By taking each sentence in the summary as an answer and feeding into our QG model, we get about 200K synthetic question-answer pairs, which are used to further pre-train the unsupervised QA model.

\subsection{Models \& Metrics}
The base model we use for both question generation and question answering tasks is BART-base~\cite{lewis-etal-2020-bart}, a widely used sequence-to-sequence framework. 

We use a suite of ROUGE~\cite{lin-2004-rouge} scores as our automatic evaluation metrics, which are also commonly used in ~\cite{fan-etal-2019-eli5,khashabi-etal-2021-gooaq-open} to examine the performance of QG and QA models. ROUGE evaluates the $n$-grams or word sequences recall of generated sentences with ground-truth sentences as references.

For our proposed QG model, we also conduct human evaluation to investigate the quality of generated questions in terms of fluency, relevance, and correctness.
% We use common metrics for assessing the performance of models for our generation tasks: ROUGE~\cite{lin-2004-rouge}, which evaluates the $n$-grams or word sequences recall of generated sentences with ground-truth sentences as references.
% BLEU~\cite{papineni-etal-2002-bleu}, METEOR~\cite{banerjee-lavie-2005-meteor}, BertScore~\cite{zhang-etal-2019-bertscore}. 
% ROUGE~\cite{lin-2004-rouge} is a recall-oriented metrics, which evaluates the $n$-grams or word sequences recall of generated sentences with ground-truth sentences as references. 
% BLEU~\cite{papineni-etal-2002-bleu} is a precision-focused metrics, which measures the average $n$-gram precision with a brevity penalty.
% METEOR~\cite{banerjee-lavie-2005-meteor} creates a word alignment between candidate and reference sentences considering stemming, paraphrases, and synonyms.
% BertScore~\cite{zhang-etal-2019-bertscore} computes cosine similarity of contextualized token embeddings between predictions and references.

\subsection{Experimental Setup}

To improve calculation efficiency, based on the dataset analysis in Section~\ref{subsec:dataset-analysis}, we set the maximum sequence length to 128 for question sentence and 256 for answer sentence.
The models are trained for 5 epochs with a learning rate of $5\times 10^{-5}$ and checkpoints are evaluated for each epoch. 
We select the checkpoint with the highest ROUGE-L score on the validation set and report its corresponding score on the test set.
Each model is run three times and average scores are recorded. 
The loss parameters $\lambda_{1}$, $\lambda_{2}$, and $\lambda_{3}$ are 1.0, 0.1, 0.1 respectively. The temperature of contrastive loss $\tau_{cl}$ is set to 0.3.


\subsection{Automatic Evaluation Results}

\smallskip
\noindent\textbf{QG performance.} The results of question generation are shown in Table~\ref{tab:qg-results}, where B represents the baseline BART-base model trained only with question generation loss, and QG represents our proposed question generator model trained with contrastive learning loss, question generation loss, and answer construction loss. It is clear that by adding a contrastive learning module and receiving feedback from the answer construction module to the question generator, the performance increases by up to 2.0\%, 2.7\%, 1.8\% on the ROUGE-L score.

\begin{table}[htbp!]
\centering\small
\begin{tabular}{cccccc}
\hline
\textbf{Dataset} & \textbf{Model} & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} & \textbf{R-Lsum} \\
\hline
\multirow{2}{*}{WikiCQA} & B & 48.39 & 26.84 & 46.08 & 46.16  \\
                         & QG & \textbf{49.22} & \textbf{27.79} & \textbf{46.98} & \textbf{47.08} \\\hline
\multirow{2}{*}{GooAQ-S} & B & 44.26 & 19.73 & 41.11 & 41.08 \\
                       & QG & \textbf{45.26} & \textbf{20.69} & \textbf{42.20} & \textbf{42.06} \\\hline
\multirow{2}{*}{ELI5} & B & 28.62 & 10.10 & 25.93 & 26.23 \\
                      & QG & \textbf{29.15} & \textbf{10.36} & \textbf{26.40} & \textbf{26.69} \\
\hline
\end{tabular}
\caption{QG results on three datasets. \texttt{B}: vanilla BART-base model; \texttt{QG}: our proposed QG model.}
\label{tab:qg-results}
\end{table}

% The contributions of each component in the proposed question generator is also investigated in the experiments.
% We can learn that by adding each module in the question generator, the performance increases.


\smallskip
\noindent\textbf{QA performance.} Taking each sentence in WikiSum summary as an answer, we use the QG model which performs best on the WikiCQA dataset to generate the question.
We use the 200K generated synthetic QA pairs to pre-train a BART closed-book QA model and validate its performance on the seen dataset (WikiCQA) and unseen datasets (GooAQ-S and ELI5).
The results are summarized in Table~\ref{tab:qa-results}. 
Without fine-tuning, our pre-trained QA model (QA) significantly outperforms the vanilla BART-base model(B) by 22.4\%, 12.5\%, and 11.4\%, on WikiCQA, GooAQ-S, and ELI5, respectively. After further fine-tuning on the target training set, our model (QA$_f$) achieves better results than B$_f$ by 3.6\%, 0.4\%, and 4.3\% on the same three datasets.
In conclusion, the consistent improvements across seen and unseen datasets indicate the good performance of our model.

% Although the vanilla BART-base model (B$_f$) fine-tuned on the target dataset outperforms our QA model (QA) in a zero-shot setting, after further fine-tuning our QA model on the target training set, our QA model (QA$_f$) achieves the best performance. The consistent improvements across seen and unseen datasets indicate the good performance of our model.

\begin{table}[htbp!]
\centering\small
\begin{tabular}{cccccc}
\hline
\textbf{Dataset} & \textbf{Model} & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} & \textbf{R-Lsum} \\
\hline
\multirow{4}{*}{WikiCQA} & B & 18.41 & 5.53 & 14.72 & 15.98 \\
                         & QA & 24.10 & 7.07 & 18.02 & 20.31 \\ \cline{2-6}
                        & B$_f$ & 27.16 & 7.32 & 19.85 & 23.49 \\                         
                         & QA$_f$ & \textbf{28.44} & \textbf{8.14} & \textbf{20.56} & \textbf{24.77} \\ \hline
\multirow{4}{*}{GooAQ-S} & B & 18.58 & 5.80 & 14.77 & 15.66 \\
                       & QA & 21.93 & 6.12 & 16.62  & 18.35 \\   \cline{2-6}                     
                       & B$_f$ & 27.72 & 7.68 & 20.08 & 23.64\\
                       & QA$_f$ & \textbf{28.44} & \textbf{7.73} & \textbf{20.17} & \textbf{24.12}  \\ \hline
\multirow{4}{*}{ELI5} & B & 12.38 & 2.19 & 8.98 & 10.63 \\
                      & QA & 13.97 & 2.29 & 10.00 & 11.77 \\   \cline{2-6}                  
                      & B$_f$ & 22.06 & 3.93 & 13.93 & 19.72 \\
                      & QA$_f$ & \textbf{23.37} & \textbf{4.27} & \textbf{14.53} & \textbf{20.88} \\
\hline
\end{tabular}
\caption{QA results on seen and unseen datasets. \texttt{B}: vanilla BART-base model without fine-tuning on the target training set; \texttt{B$_f$}: vanilla BART-base model fine-tuned on the target training set; \texttt{QA}: our unsupervised QA model without fine-tuning on the target training set; \texttt{QA$_f$}: our unsupervised QA model further fine-tuned on the target training set.}
\label{tab:qa-results}
\end{table}
\vspace{1ex}

\subsection{Human Evaluation}
We additionally perform human evaluations to measure the quality of questions generated by our system.
We randomly sample 100 question-answer pairs from the WikiCQA dataset and ask three annotators to rate the generated questions from the baseline model and our best model.
The questions are rated on a 1-5 scale (5 for the best) from the following aspects: (1) fluency: whether the questions are grammatically correct and fluent; 
(2) relevance: whether the question is related to the answer; and 
(3) correctness: whether the question can be answered by the answer.
The average scores with the inter-annotator agreement -- Fleiss' $\kappa$ score -- are shown in Table~\ref{tab:human-evaluation}.
We can see our approach performs better than the baseline method in terms of relevance and correctness with fair agreement among raters.


\begin{table}[htbp!]
\centering\small
\begin{tabular}{ccccccc}
\hline
\multirow{2}{*}{Model} & \multicolumn{2}{l}{fluency} & \multicolumn{2}{l}{relevance} & \multicolumn{2}{l}{correctness}  \\
                       & score & $\kappa$ & score & $\kappa$ & score & $\kappa$ \\ 
\hline
B & 4.83 & 0.39 & 3.84 & 0.41 & 3.49 & 0.38                         \\
QG & 4.83 & 0.38 & \textbf{3.89} & 0.40 & \textbf{3.58} & 0.42  \\
\hline
\end{tabular}
\caption{Human evaluation.}
\label{tab:human-evaluation}
\end{table}


% Cohen's kappa K
% From the table we can see, our approach performs better than the baseline in terms of these three aspects. In addition, for our model, the inter-annotator agreement shows moderate or good agreement between raters.





==> tex/introduction.tex <==
\section{Introduction}

As a critical topic in Natural Language Processing, Question Answering (QA) has a wide range of applications in intelligent conversational systems (e.g., chatbots and voice assistants), education~\cite{jia-etal-2021-eqg}, and health~\cite{he-etal-2020-infusing}, attracting lots of attention in recent years.
The QA task focuses on training a model to retrieve or generate the answer to a given question.
Most past work targets reading comprehension QA datasets (e.g., SQuAD~\cite{rajpurkar-etal-2016-squad}), where question-context pairs are fed into the model to extract the short answer span in context. This \textit{open-book} setting is modeled after open book exams, where the model has access to resources (like the context here) to find a good answer. Different from the open-book QA task, \textit{closed-book} Question Answering challenges models to answer questions without accessing any external knowledge or context~\cite{roberts-etal-2020-much}.
% These models are directly fine-tuned on question-answer pairs and rely on the information stored in their parameters to answer the questions.
This closed-book setting is appealing in practice since labeling question-context pairs requires a large amount of time and human effort.

Question Generation (QG) is a dual task of QA, which can be leveraged as a data augmentation strategy to create large-scale QA pairs to improve the performance of a QA model. Like open-book QA, most QG frameworks also mainly focus on reading comprehension datasets, and the questions are usually generated from factoid short answers or the sentence containing the answer with the corresponding passages~\cite{du-etal-2017-learning, zhao-etal-2018-paragraph}.
However, due to the lack of corresponding passages in closed-book data, existing open-book QG approaches can not be directly applied to the closed-book setting.
In this work, we propose a novel question generator under the closed-book setting to bridge this gap.

Two of the unique characteristics of the proposed model are: (i) a contrastive learning loss designed to learn a better question representation; and (ii) an answer reconstruction loss designed to measure the answerability of the generated question. Contrastive learning has shown promising results in many NLP tasks, e.g., ~\cite{giorgi-etal-2021-declutr, gao-etal-2021-simcse}; here we show how to learn question representations by distinguishing features of correct QA pairs from features of incorrectly linked QA pairs. Further, we frame the model as a generation-reconstruction process through the use of a pre-trained seq2seq model to predict the original answer given the generated question (see Section~\ref{sec:approach}). Figure~\ref{fig:pipeline} shows our synthetic QA data generation framework and generated question examples from our QG model.
\begin{figure*}[htbp!]
\centering
\includegraphics[width=\linewidth]{img/pipeline.pdf}
\caption{An overview of synthetic data generation framework and generated question examples from our QG model. Taking each sentence from the summary as an answer, our trained QG model is employed to generate the question.}    
\label{fig:pipeline}
\end{figure*}
In addition, we introduce a new closed-book dataset with abstractive long answers -- WikiCQA -- based on question-answer pairs from WikiHow, a wiki-style website featuring over 200K how-to articles. Questions like ``What can I feed my dog if I have run out of dog food?'' result in long (non-factoid) answers crafted by  knowledgeable WikiHow users or editors. WikiCQA complements existing datasets like GooAQ~\cite{khashabi-etal-2021-gooaq-open} and ELI5~\cite{fan-etal-2019-eli5} by providing abstractive long answers appropriate for the closed-book setting.

Through experiments, we find the proposed QG model shows significant improvement through both automatic and human evaluation metrics on these three datasets. Compared with the vanilla BART-base model, our QG model shows improvement of up to 2.0\%, 2.7\%, and 1.8\% on the ROUGE-L score on WikiCQA, GooAQ-S, and ELI5, respectively.
% \textcolor{blue}{CAV: can you show some percentage improvement? or mention some specific numbers here?} 
We further evaluate our QG model by employing it to generate synthetic QA data from WikiHow summary data to pre-train a closed-book QA model in an unsupervised setting and evaluate the performance on both seen (WikiCQA) and unseen (GooAQ-S, ELI5) datasets, where we find the consistent improvements across these datasets, which indicates the good performance of our model.

In conclusion, our contributions can be summarized as follows:
\squishlist
\item We propose a closed-book QG model, which to our knowledge is the first work to explore QG under a closed-book setting based on a dataset with abstractive long answers.
\item We present a new closed-book dataset with abstractive long answers -- WikiCQA -- of 20,202 real user QA pairs collected from WikiHow. 
In addition, we show that WikiCQA is a valuable training resource for both Closed-Book QA and QG tasks.
\item We employ our QG model to generate synthetic QA data from WikiHow article summaries to pre-train the Closed-Book QA model, which achieves the best performance on the seen dataset and shows strong generalization on unseen datasets.
\squishend

%besides existing datasets, GooAQ~\cite{khashabi-etal-2021-gooaq-open} and ELI5~\cite{fan-etal-2019-eli5}, we also present a new closed-book dataset with abstractive long answers, WikiCQA, to train it (Section~\ref{sec:dataset}).
%To help our model learn a better question representation, we apply contrastive learning into it and frame the model as a generation-reconstruction process, which is described in detail in Section~\ref{subsec:qg}.

% As a dual task of QA, most QG frameworks also mainly focus on reading comprehension datasets with short answers either as text spans within paragraphs (e.g., SQuAD~\cite{rajpurkar-etal-2016-squad}, NewsQA~\cite{trischler-etal-2017-newsqa}, HotpotQA~\cite{yang-etal-2018-hotpotqa}) or human-generated short answers (e.g., Narrative QA~\cite{kocisky-etal-2018-narrativeqa}), the questions are usually generated from factoid short answers or the sentence containing the answer with the corresponding passages~\cite{du-etal-2017-learning, zhao-etal-2018-paragraph}.

% Although fine-tuning pre-trained language models (e.g., BERT~\cite{devlin-etal-2019-bert}, BART~\cite{lewis-etal-2020-bart}) on large amounts of labeled QA datasets shows significantly advances in extractive QA task, the Closed-Book QA performance is still poor.
% One of the challenges is that collecting such labeled training data requires significant cost and resources.
% A common approach is through synthetic data generation, which demonstrates success in improving the downstream extractive QA task~\cite{alberti-etal-2019-synthetic, puri-etal-2020-training}.
% Some recent approaches for synthetic QA data generation based on large pre-trained language models have started to demonstrate success in improving the downstream extractive QA task~\cite{alberti-etal-2019-synthetic, puri-etal-2020-training}.
% Typically, these work utilize the passage to extract text span as answers via heuristics and then feed answer-context pairs to train a QG model. 
% Then, the synthetic question-passage-answer pairs are used to improve model performance on QA task.

% These approaches typically consist of multiple stages: span/answer extraction, question generation, and question filtering. 


% Question Generation (QG) gains increasingly attention in recent years from both academic and industrial communities. It has huge potential benefits to various fields. As a dual task of question answering, QG can be leveraged as a data augmentation strategy to create large-scale question-answer pairs to improve the performance of a QA model. In addition, QG can be useful in conversational systems, such as Alexa and Siri, which can help them interact with humans better. Moreover, QG can be used in education area to generate quiz questions.


==> tex/other.tex <==
\cite{mishra-etal-2020-towards}
In addition, long-answer setting where the target answer spans 4 or more sentences on average but on NQ (~\cite{kwiatkowski-etal-2019-natural} where the answers are paragraph from the relevant Wikipedia page.

==> tex/related-work.tex <==
\section{Related Work}

\smallskip
\noindent\textbf{Question Answering} (QA) and \textbf{Question Generation} (QG) are two core tasks in Natural Language Processing (NLP) area. QA focuses on training a model to retrieve or generate the answer for a given question.
Most QA works provide the model with additional contexts that contain or support the answer alongside the question, which is referred to as the ``open-book'' QA.
Different from open-book QA, closed-book QA does not allow the model to access any external knowledge~\cite{roberts-etal-2020-much}.
As a dual task of open-book QA, QG models take factoid short answers (e.g., SQuAD~\cite{rajpurkar-etal-2016-squad}) or human-generated short answers (e.g., Narrative QA~\cite{kocisky-etal-2018-narrativeqa}) with the corresponding passages to generate questions~\cite{zhang-etal-2021-review}.
% As a dual task of open-book QA, most QG frameworks target reading comprehension datasets with short answers either as text spans within paragraphs (e.g., SQuAD~\cite{rajpurkar-etal-2016-squad}, NewsQA~\cite{trischler-etal-2017-newsqa}, HotpotQA~\cite{yang-etal-2018-hotpotqa}) or human-generated short answers (e.g., Narrative QA~\cite{kocisky-etal-2018-narrativeqa}),
% the efforts in QG usually seek to generate natural questions relevant to the input which contains the input context text and optionally a specific target answer~\cite{zhang-etal-2021-review}.
Early approaches for question generation rely on rule-based methods~\cite{labutov-etal-2015-deep, khullar-etal-2018-automatic}. To bypass hand-crafted rules and sophisticated NLP pipelines in QG, researchers in ~\citet{du-etal-2017-learning} introduce a vanilla RNN-based sequence-to-sequence approach with an attention mechanism. The pre-trained transformer-based frameworks proposed recently, including BART~\cite{lewis-etal-2020-bart} and T5~\cite{raffel-etal-2020-exploring}, also move forward the performance of QG. 
However, their success can not directly carry over to the closed-book setting, where the model is supposed to generate questions solely relying on answers.
In our work, we explore closed-book QG, which is a widely applicable setting and has not been investigated.


% \textcolor{blue}{CAV: this is an important paragraph! Need to add a sentence at the end explaining how we are different.}

% However, since most QG frameworks target reading comprehension datasets with short answers either as text spans within paragraphs (e.g., SQuAD~\cite{rajpurkar-etal-2016-squad}, NewsQA~\cite{trischler-etal-2017-newsqa}, HotpotQA~\cite{yang-etal-2018-hotpotqa}) or human-generated short answers (e.g., Narrative QA~\cite{kocisky-etal-2018-narrativeqa}),
% their success can not directly carry over to the closed-book setting
% the questions are usually generated from factoid short answers or the sentence containing the answer with the corresponding passages~\cite{du-etal-2017-learning, zhao-etal-2018-paragraph}.


% \textcolor{blue}{CAV: another important paragraph! But here the emphasis seems to be on open-book. Need to be clear about the differences -- e.g., open-book and separately long-form abstractive answers. These are related but different points. Need to make them crystal clear.}

% Instead of following the open-book setting in previous works to provide the access to external knowledge and context text, we focus on the closed-book setting~\cite{roberts-etal-2020-much}) with long-form abstractive answers~\cite{fan-etal-2019-eli5}, which is a more practical setting and has not been investigated in QG task.



%However, by not allowing the model to access any external knowledge, \citet{roberts-etal-2020-much} proposed closed-book question answering.
%Thus, the QG task under closed-book setting has not been fully investigated.

\smallskip
\noindent\textbf{Contrastive Learning} aims to seek a representation space in which semantically similar neighbors are close and non-neighbors are far apart, and has achieved great success under both supervised and unsupervised settings. 
In pioneer works, the contrastive loss function \cite{hadsell2006dimensionality,chopra2005learning} has been proposed as a training objective in deep metric learning considering both similar and dissimilar pairs. Recently,  \citet{chen-etal-2020-simple} proposes a simple framework SimCLR with the exploration in data augmentation, encoder, projection head, and loss function of contrastive learning for visual representations. Viewing contrastive learning as dictionary look-up, Momentum Contrast (MoCo) \cite{he-etal-2020-momentum} proposes to build a dynamic dictionary and a moving-averaged encoder, which can be large and consistent as they evolve during the training process. 
% Among the recent efforts in natural language processing building on top of contrastive learning for sentence representation,  
% \citet{pan-etal-2021-contrastive} proposes to use a contrastive learning scheme to reduces the gap of different language representations multilingual neural machine translation. 
% In ConSERT \cite{yan-etal-2021-consert}, a contrastive framework is presented to solve the collapse issue of BERT-derived sentence representations for self-supervised sentence representation transfer. 
There are also some works trying to apply contrastive learning into the natural language processing domain to learn better sentence representations~\cite{giorgi-etal-2021-declutr, gao-etal-2021-simcse}.
In addition, contrastive learning has been applied in paraphrase generation~\cite{yang-etal-2021-contrastive-representation}, multilingual neural machine translation~\cite{pan-etal-2021-contrastive}, abstractive summarization~\cite{liu-liu-2021-simcls}, and multi-document question generation~\cite{cho-etal-2021-contrastive}.
In this work, we propose to adopt contrastive learning for improving representation learning in question generation under a closed-book setting.  

\smallskip 
\noindent \textbf{Synthetic QA Data Generation} typically consist of multiple stages: answer extraction, question generation, and question filtering~\cite{alberti-etal-2019-synthetic, puri-etal-2020-training}.
For a given passage, the responsibility of the answer extractor is to extract appropriate spans that will serve as answers to generate questions. 
Usually, question (un)conditional extractive answer models~\cite{alberti-etal-2019-synthetic, puri-etal-2020-training} or heuristics (e.g., noun phrases, named entities)~\cite{lewis-etal-2019-unsupervised, lyu-etal-2021-improving} are used in this module.
Then, questions are generated conditioned on passages and answers.
After that, the questions are filtered based on the roundtrip consistency.
To reduce the errors propagated from each module to others in the pipeline, \citet{shakeri-etal-2020-end} proposed an end-to-end approach for synthetic QA data generation.

Since freely available summary data is a good resource to generate synthetic data~\cite{lyu-etal-2021-improving}, we also explore synthetic data generation for the closed-book QA task based on summary data.




% However, these works are all performed on reading comprehension datasets which is different from the closed-book setting.
% \textcolor{blue}{CAV: need to talk about our naming conventions ... here it is "closed-book long-form" ... are we consistent? and we should carefully introduce what we mean by long form earlier in the paper (and contrast with the other kind ... the factoid/short kind, maybe with an example)}

